Ab initio Study of Aspirin Adsorption on Single-walled Carbon and Carbon Nitride Nanotubes

We use ab intio density functional theory to investigate the adsorption properties of acetylsalicylic acid or aspirin on a (10, 0) carbon nanotube (CNT) and a (8, 0) triazine-based graphitic carbon nitride nanotube (CNNT). It is found that an aspirin molecule binds stronger to the CNNT with its adsorption energy of 0.67 eV than to the CNT with 0.51 eV. The stronger adsorption energy on the CNNT is ascribed to the high reactivity of its N atoms with high electron affinity. The CNNT exhibits local electric dipole moments, which cause strong charge redistribution in the aspirin molecule adsorbed on the CNNT than on the CNT. We also explore the influence of an external electric field on the adsorption properties of aspirin on these nanotubes by examining the modifications in their electronic band structures, partial densities of states, and charge distributions. It is found that an electric field applied along a particular direction induces aspirin molecular states in the in-gap region of the CNNT implying a potential application of aspirin detection.

==> howtocomment.tex <==
\towho[inline,caption={To All Authors: Put your comment in this way}]
{All Authors}{If you want to give a commment, put your comment in this
way (Replace italic words by your own word, while keeping the others as they are):
  \begin{itemize}\setlength\itemsep{-\parsep}
     \item For comments on side margin, use \\
       {\tt{{\textbackslash}mycomment\{{\it{ABC}}\}\{{\it{Your comment}}\}}}, \\
       where {\it{ABC}} is your initial, e.g., YKK for Young-Kyun Kwon
     \item For inline comments, use \\
       {\tt{{\textbackslash}mycomment[inline]\{{\it{ABC}}\}\{{\it{Your comment}}\}}}
     \item If you want to put itemized list in your comment, use \\
       {\tt{{\textbackslash}mycomment[inline,caption=\{{\it{a short comment for Todo list}}\}]\{{\it{ABC}}\} \\
       \{{\it{A short comment giving an explanation of list if needed}} \\
       \quad{\textbackslash}begin\{itemize\}
         {\textbackslash}setlength{\textbackslash}itemsep\{-{\textbackslash}parsep\} \\
       \quad\quad{\textbackslash}item {\it{your comment 1}} \\
       \quad\quad{\textbackslash}item {\it{your comment 2}} \\
       \quad\quad{\textbackslash}item {\it{your comment 3}} \\
       \quad{\textbackslash}end\{itemize\} \}}} \\
       For enumerated list, substitute {\tt{itemize}} in both
       {\tt{{\textbackslash}begin\{itemize\}}} and 
       {\tt{{\textbackslash}end\{itemize\}}} with {\tt{enumerate}}
  \end{itemize}
}

==> todopreamble.tex <==
\usepackage[obeyFinal,colorinlistoftodos]{todonotes}

\setlength{\marginparwidth}{2cm}
\newcommand{\todoin}[2][]{\todo[inline,#1]{#2}}
\newcommand{\towho}[3][]{\todo[color=red!60,#1]{To #2: #3}}
\newcommand{\addref}{\todo[color=green!40,fancyline]{Add reference!}}

\newcounter{comm}
\newcommand{\mycomment}[3][]{
  \refstepcounter{comm}
  \todo[color=blue!60!green!20,size=\small,#1]{{\textbf{[#2\thecomm]: }}#3}
}
